Change Patterns in Use: A Critical Evaluation

Process model quality has been an area of considerable research efforts. In this context, the correctness-by-construction principle of change patterns provides promising perspectives. However, using change patterns for model creation imposes a more structured way of modeling. While the process of process modeling (PPM) based on change primitives has been investigated, little is known about this process based on change patterns. To obtain a better understanding of the PPM when using change patterns, the arising challenges, and the subjective perceptions of process designers, we conduct an exploratory study. The results indicate that process designers face little problems as long as control-flow is simple, but have considerable problems with the usage of change patterns when complex, nested models have to be created. Finally, we outline how effective tool support for change patterns should be realized.

==> backgrounds.tex <==
\section{Backgrounds}
\label{backgrounds}
This section first introduces cognitive foundations of the PPM (cf.
Sect.~\ref{cognFound}) and presents backgrounds on the PPM when using
change primitives (cf. Sect.~\ref{PPM}) before turning to model creation based on change
patterns (cf. Sect.~\ref{patternsVersusPrimitives}).  
% Finally, Sect.
% \ref{measuringDifferences} discusses the measurment of differences between process models.
 
\subsection{Cognitive Foundations of Problem Solving}\label{cognFound}
We consider the creation of process models to be a complex problem solving task.
Problem solving has been an area of vivid research in cognitive
psychology for decades. Therefore, we turn to cognitive psychology to understand
the processes followed by humans when solving a problem like creating a process model.
  

\textbf{Schemata.} A central insight from cognitive research is that the human
brain contains specialized regions contributing different functionality to the
process of \emph{solving complex problems}. \emph{Long-term memory} is
responsible for permanently storing information and has an essentially unlimited
capacity, while in \emph{working memory} comparing, computing and reasoning take
place~\cite{Gray07}. Although the latter is the main working area of the brain, it can store only a limited amount of information, which is forgotten after 20--30
seconds if not refreshed~\cite{Trac79}. The question arises how information can
be processed with such limited capacity. The human mind organizes information in
interconnected \emph{schemata} rather than in isolation~\cite{Gray07}. Those
schemata, stored in long-term memory, incorporate general concepts of similar
situations~\cite{Gray07}. Whenever situations similar to a schema arise, the
latter is retrieved to help organizing information by creating \emph{chunks} of
information that can be processed efficiently~\cite{JTPA81}. For instance, when
asked to create a process model using change patterns, a designer must create an
internal representation of the problem~\cite{Sof+12}. For this, information about
the domain is retrieved and organized in memory using existing schemata for
process modeling. Therefore, schemata guide the comprehension process, helping to
re-organize information for its processing in working memory~\cite{JTPA81}.



 
\textbf{Problem-Solving Strategies.} When
confronting novices with an unfamiliar problem they cannot rely on specialized
problem solving strategies. Instead, they must find a way to solve the problem
and come up with an initial skeletal \emph{plan}~\cite{Rist89}. Then, novices
utilize general problem solving strategies, like means-ends analysis, due to
the lack of more specific strategies for the task at hand~\cite{KaNe84}.
Means-ends analysis can be described as the continual comparison of the problem's current
state with the desired end product. Based on this, the next steps are selected until a
satisfying solution is found~\cite{KaNe84}. After applying the constructed plan,
it can be stored in long-term memory as \emph{plan schema}~\cite{Rist89}. For
this, task-specific details are removed from the plan schema resulting in a plan
schema that can be automatically applied in similar situations~\cite{Ande82}.
When confronted with a problem solving task in the future, the appropriate plan
schema is selected using a case-based reasoning approach~\cite{GuCu88}. The
retrieved plan schema provides the user with structured knowledge
that drives the process of solving the problem~\cite{JTPA81,GuCu88}. Plan
schemata allow experts to immediately decide what steps to apply to end up with
the desired solution~\cite{Swel88}. If the plan schema is well developed, an
expert never reaches a dead end when solving the problem~\cite{Broo77}.


 
Plan schemata seem to be important when creating process models based on change
patterns since change pattern cannot be combined in an arbitrary manner. If no
plan schema is available on how to combine change patterns to create the desired
process model, designers have to utilize means-ends analysis until a satisfying
solution is found. This behavior is more likely to reach in detours, reducing the
process designer's efficiency when creating process models. 


\subsection{The Process of Process Modeling}\label{PPM}
During the formalization phase, process designers create a syntactically correct
process model reflecting a given domain description by interacting with the
process editor~\cite{HoPW05}. The formalization, i.e., the PPM, can be described
as a cycle of the three phases of comprehension, modeling and
reconciliation~\cite{PZW+12,Sof+12}.


  
\textbf{Comprehension.} In comprehension phases designers try to understand the
requirements to be modeled by extracting information from the task description
and the existing process model to build an internal representation of the problem
in working memory~\cite{KaNe84,Broo77}. Depending on the availability of schemata
for organizing the acquired knowledge, working memory is utilized more or less
efficiently. If the process designer has solved a similar problem previously
(i.e., a plan schema for the problem is stored in long-term memory), the designer
can directly create the process model without any further attention on which
steps to execute or plan next, which puts an additional burden on designers by
occupying cognitive resources. Either way, working memory is filled with
knowledge extracted from requirements and, if available, the process model being
created.

 

\textbf{Modeling.} The designer uses the internal representation
developed during the comprehension phase to materialize the solution in a process
model (by creating or changing it)~\cite{Sof+12,PZW+12}. Hence, modeling phases
consist of a set of structural model adaptations. More specifically, designers
interact with the modeling environment using change primitives such as {\tt add
activity} or {\tt add edge}. The materialization of a process model adaptation
may require the joint application of several change primitives. For instance,
when adding an activity to the process model, the newly created activity and the
edges connecting it with the process model must be created. Once all information
stored in working memory is incorporated in the process model, the designer
interrupts the modeling endeavor to incorporate additional requirements into the
internal representation~\cite{PZW+12}.

 

 

\textbf{Reconciliation.} Designers may reorganize a process model (e.g.,\
renaming of activities) and utilize its \emph{secondary notation} (e.g.,\
notation of layout, typographic cues) to enhance understandability~\cite{Petr95}. However, the
number of reconciliation phases in the PPM depends on the designer's ability
of placing elements correctly when creating them~\cite{PZW+12}.
 
\vspace{-0.2cm}

\subsection{Process Modeling Based on Change Patterns}
\label{patternsVersusPrimitives}
Change patterns provide a different way of interacting with the modeling
environment in modeling phases. Instead of specifying a set of change primitives,
the process designer applies change patterns (i.e., high-level change operations)
to realize the desired model adaptation. Examples of change patterns include the
insertion and deletion of process fragments, or their embedding in loops. The
whole catalogue of change patterns can be found in
\cite{DaRe09,WRR08}, while the semantics of these patterns
are described in \cite{DBLP:conf/er/Rinderle-MaRW08}. When applying a single
change primitive, soundness of the resulting process model cannot be guaranteed,
but must be explicitly checked after applying the change primitives. On the
contrary, change pattern implementations often associate pre-/post-conditions
with high-level change operations to guarantee model correctness after each
adaptation \cite{ReDa98,Casa98}. Process editors applying the
correctness-by-construction principle (e.g., \cite{DaRe09})
usually provide only those change patterns to the process designer that allow
transforming a sound process model into another sound one. This is realized by
imposing structural restrictions on process models (e.g., block structurdness).



% 
% \begin{definition}[Structural Model Change]
% \label{def:structural_change}
% Let $\cal{P}$ be the set of all process models and let $S$, $S' \in \cal{P}$. Let
% further $\Delta=(op)$ $\in \mathcal{C}$ denote a particular change consisting of
% one change operation $op$ and $\tau$= $<op_1, ..., op_n>$ $\in \mathcal{C^*}$ be
% a process change that applies change operations $op_i$, i=1,\ldots,n
% sequentially.
% \begin{enumerate}
% \item $S$ $[\Delta\rangle$ iff $\Delta$ is applicable to $S$
% \item $S$ $[\Delta\rangle$ $S'$ iff $\Delta$ is applicable to $S$ (i.e., $S$ $[\Delta\rangle$) and $S'$ is the process model resulting from the application of $\Delta$ to $S$ (also: $S'=S+\Delta$)
% \item $S$ $[\tau\rangle$ $S'$ iff there are process models $S_1,S_2$,\ldots
% $S_{n+1}$ $\in \cal{P}$ with $S=S_1,S'=S_{n+1}$ and for 1 $\leq$ i $\leq$ n: $S_i$ $[\Delta_i\rangle$ $S_{i+1}$ with $\Delta_i = (op_i)$
% \end{enumerate}
% \end{definition}





% \subsection{Measuring Differences Between Process
% Models}\label{measuringDifferences} Change pattern can be utilized for measuring
% differences between process models. The difference between an original process model (in terms of change patterns)
% and a modified one is denoted as \textit{bias}~\cite{ReWe12}. Given a certain set
% of high-level change operations, the \emph{distance} between process models $S$
% and $S'$ corresponds to the minimum number of concrete change operations needed
% for transforming $S$ into $S'$. The corresponding sequence of change operations
% is denoted as \emph{bias} $B_{S,S'}$. Generally, there may be more than one minimum set of change operations
% transforming $S$ into $S'$ (i.e., a bias does not have to be unique). Inserting
% the fragment depicted in Fig. \ref{img:tasksA+B} starting from an empty
% modeling canvas can be achieved in several different ways with a minimum
% number of 4 change patterns. For
% example, model $S'$ can be created by first inserting region \textit{R4.1}, next
% embedding region \textit{R4.1} in a conditional branch, then
% inserting activity \textit{R4.2}, and finally updating the edge condition.
% 
% \begin{definition}[Bias and Distance]
% \label{def:bias_distance}
% Let $S$, $S' \in \cal{P}$ be two process models and let $\mathcal{C^*}$ be the
% set of all potential changes (i.e., sequences of change operations). Then:
% \textbf{Distance} $d_{(S,S')}$ between $S$ and $S'$ corresponds to the minimal
% number of high-level change operations needed to transform $S$ into $S'$; i.e.,
% we define
% \begin{equation}
% d_{(S,S')}= \min\{|\tau| \hspace{1mm} \big| \hspace{1mm} \tau \in
% \mathcal{C^*} \wedge S[\tau\rangle S'\}
% \end{equation}
% Furthermore, a sequence of change operations $\tau$ with $S[\tau\rangle S'$
% and $|\tau| = d_{(S,S')}$ is denoted as \textbf{bias} between $S$ and $S'$
% ($B_{S,S'}$ for short).
% \end{definition}


 
% Generally, there may be more than one minimum set of change operations
% transforming $S$ into $S'$ (i.e., a bias does not have to be unique). Inserting
% the fragment depicted in Fig. \ref{fig:structuralChange} starting from an empty
% modeling canvas can be achieved in several different ways. Each path through
% this model has a distance of 4 and shows one alternative to construct this
% fragment with the minimum number of change operations (i.e., depictes one
% possible \textit{bias}). For example, model $S'$ can be created by first inserting
% activity \textit{Announce Taxiing}, next embedding activity \textit{Announce Taxiing} in a conditional branch, then inserting activity \textit{Contact Ground} and finally
% updating the edge condition. 

% \begin{figure}[h!tb]
% \center
%   \includegraphics[width=1\textwidth]{StructuralChange}
%   \caption{Different Alternatives for Constructing a Process Fragment}
%   \label{fig:structuralChange}\par\vspace{\textfloatsep} 
%   \center
% \end{figure}
% 
% \todo{it just takes to much space; any ideas how to present this differently?}
% 
% \todo{redraw figure}





